Price Competition in Online Combinatorial Markets

We consider a single buyer with a combinatorial preference that would like to purchase related products and services from different vendors, where each vendor supplies exactly one product. We study the general case where subsets of products can be substitutes as well as complementary and analyze the game that is induced on the vendors, where a vendor's strategy is the price that he asks for his product. This model generalizes both Bertrand competition (where vendors are perfect substitutes) and Nash bargaining (where they are perfect complements), and captures a wide variety of scenarios that can appear in complex crowd sourcing or in automatic pricing of related products. We study the equilibria of such games and show that a pure efficient equilibrium always exists. In the case of submodular buyer preferences we fully characterize the set of pure Nash equilibria, essentially showing uniqueness. For the even more restricted "substitutes" buyer preferences we also prove uniqueness over {\em mixed} equilibria. Finally we begin the exploration of natural generalizations of our setting such as when services have costs, when there are multiple buyers or uncertainty about the the buyer's valuation, and when a single vendor supplies multiple products.

==> pricing-competition-multiple.tex <==
\mbcomment{the paper uses $m$ for the number for agents, and $n$ for the number of items. We need to change the notation below to be consistent with this.}
\mbcomment{How do you find $k$ ?}
\mbcomment{How to compute expectations. Be explicit about with high probability.}

\begin{lemma}
Let $v$ be an arbitrary valuation on $m$ items then there exists a set $S$ such that
$\sum_{j \in S}v(j|S-j) \ge v([m])/H_m$, where $H_m = \sum_{i=1}^m i^{-1}= \Theta(\log m)$ is
the $m$'th harmonic
number.  Furthermore a set $S$ with $\sum_{j \in S}v(j|S-j) = \Omega(v([m])/\log m)$ can be found in
(randomized) polynomial time.
\end{lemma}

\begin{proof}
Let us first prove the lemma for symmetric valuations, i.e. where for each set $S$ of size $k$ we have
$v(S)=v(k)$.  Define $\Delta_k=v(k)-v(k-1)$ and so we have $v(m)=\sum_{k=1}^m \Delta_m$ and
for $|S|=k$ we have
$\sum_{j \in S}v(j|S-j) = k \cdot \Delta_k$.  Thus we need to show that for some $1 \le k \le m$ it holds that
$k \cdot \Delta_k \ge v(m)/H_m$.  Otherwise, we have $\Delta_k < k^{-1} v(m)/H_m$ for all $k$ and so
$v(m)=\sum_{k=1}^m \Delta_k < (\sum_{k=1}^m k^{-1}) v(m)/H_m = v(m)$, a contradiction.

Now let us prove the lemma for arbitrary, not necessarily symmetric $v$'s.  Let us look at the
symmetrization of $v$, $\tilde{v}(k) = E_{|S|=k} v(S)$.  Note that $\tilde{v}(m) = v([m])$ and
when we define $\Delta_k=\tilde{v}(k)-\tilde{v}(k-1)$, we have that
$k\cdot\Delta_k = E_{|S|=k} \sum_{j \in S}v(j|S-j)$.  So, for the $k$ that has
$k \cdot \Delta_k \ge \tilde{v}(m)/H_m = v([m])/H_m$,
we have that in expectation over the sets $S$ of size $k$ it holds that
$\sum_{j \in S}v(j|S-j) \ge v([m])/H_m$.
We can find a set $S$ with close to that value by looking for it randomly among all sets of size $k$.
Such a search can not require more than $O(m\log m)$ samples since we clearly have the upper bound
$\sum_{j \in S}v(j|S-j) \le m \cdot v([m])$ so at least $\Omega(1/(m\log m))$ fraction of $S$'s must have
$\sum_{j \in S}v(j|S-j)$ above $v([m])/(2H_m)$.
\end{proof}

This lemma is best possible even for symmetric downward sloping (and thus GS) valuations as can be seen
by the valuation $v(k)=H_k$ which has $\sum_{j \in S}v(j|S-j) = 1$ for all sets $S$,
while $v(m)=\Theta(\log m)$.



